Vita-CLIP: Video and text adaptive CLIP via Multimodal Prompting

Adopting contrastive image-text pretrained models like CLIP towards video classification has gained attention due to its cost-effectiveness and competitive performance. However, recent works in this area face a trade-off. Finetuning the pretrained model to achieve strong supervised performance results in low zero-shot generalization. Similarly, freezing the backbone to retain zero-shot capability causes significant drop in supervised accuracy. Because of this, recent works in literature typically train separate models for supervised and zero-shot action recognition. In this work, we propose a multimodal prompt learning scheme that works to balance the supervised and zero-shot performance under a single unified training. Our prompting approach on the vision side caters for three aspects: 1) Global video-level prompts to model the data distribution; 2) Local frame-level prompts to provide per-frame discriminative conditioning; and 3) a summary prompt to extract a condensed video representation. Additionally, we define a prompting scheme on the text side to augment the textual context. Through this prompting scheme, we can achieve state-of-the-art zero-shot performance on Kinetics-600, HMDB51 and UCF101 while remaining competitive in the supervised setting. By keeping the pretrained backbone frozen, we optimize a much lower number of parameters and retain the existing general representation which helps achieve the strong zero-shot performance. Our codes/models are released at https://github.com/TalalWasim/Vita-CLIP.

==> tables/ablations/num_global_prompts.tex <==
\begin{table}[t!]
% \vspace{-.4cm}

\caption{Ablations for number of Global video-level prompts ($\mathbf{G}^{(l)} = [\mathbf{g}_{1}^{(l)}, \cdots, \mathbf{g}_{M_v}^{(l)}]$) on Kinetics-400. The video-side prompting includes Local frame-level prompting ($L$) and summary token ($S$). Text side prompting is fixed to $M_c = 8$.}
\centering
\small
\setlength{\tabcolsep}{1.0mm}{
\begin{tabular}{lc} 
\rowcolor{Gray}
\toprule
	Method             & Top-1 \\
    \midrule
	Vita-CLIP B/16 $L$ + $S$ + $G$ ($M_v = 5$)     & 79.80 \\
    Vita-CLIP B/16 $L$ + $S$ + $G$ ($M_v = 8$)     & 80.51 \\
	Vita-CLIP B/16 $L$ + $S$ + $G$ ($M_v = 10$)    & 80.62 \\
	Vita-CLIP B/16 $L$ + $S$ + $G$ ($M_v = 15$)    & 80.71 \\
    Vita-CLIP B/16 $L$ + $S$ + $G$ ($M_v = 25$)    & 80.92 \\
    \bottomrule
\end{tabular}
}

\label{tab:ablation_num_global}
\hfill

\end{table}

==> tables/ablations/type_num_text_prompts.tex <==
\begin{table}[t!]
% \vspace{-.4cm}

\caption{Ablations for the number of text prompts ($M_c = 8$, $M_c = 16$, $M_c = 32$) and type of text prompts (Unified Context (UC) vs Class-Specific Context (CSC), on Kinetics-400, supervised training. Vision-side prompting is fixed to global video-level prompting $M_v = 8$ with local frame-level prompting  and summary token.}
\centering
\small
\setlength{\tabcolsep}{1.0mm}{
\resizebox{0.4\columnwidth}{!}{
\begin{tabular}{lc}
\rowcolor{Gray}
\toprule
	Method             & Top-1 \\
    \midrule
	UC ($M_c = 8$)     & 78.97 \\
	UC ($M_c = 16$)    & 79.12 \\
	UC ($M_c = 32$)    & 79.33 \\
	CSC ($M_c = 8$)    & 80.51 \\
	CSC ($M_c = 16$)   & 80.46 \\
	CSC ($M_c = 32$)   & 80.56 \\
    \bottomrule
\end{tabular}
}
}
\label{tab:ablation_text}
\hfill
\end{table}
